PLUM: Improving Inference Efficiency By Leveraging Repetition-Sparsity Trade-Off

Efficient inference of Deep Neural Networks (DNNs) on resource-constrained edge devices is essential. Quantization and sparsity are key techniques that translate to repetition and sparsity within tensors at the hardware-software interface. This paper introduces the concept of repetition-sparsity trade-off that helps explain computational efficiency during inference. We propose PLUM, a unified co-design framework that integrates DNN inference systems and quantization (forward and backward pass) to leverage the repetition-sparsity trade-off to improve inference efficiency. Our results demonstrate that PLUM's quantization method is more accurate than binary quantization with the same number of non-zero weights. Detailed analysis indicates that signed binarization generates a smaller distribution of effectual (non-zero) parameters nested within a larger distribution of total parameters of latent full-precision weights for a DNN block. Finally, the proposed PLUM framework achieves a 26% speedup on real hardware, doubles energy efficiency, and reduces density by 2.8x compared to binary methods while retaining top-1 accuracy when compared to prior-art methods for ResNets on ImageNet (by achieving 66.2% top-1 accuracy), presenting an alternative solution for deploying efficient models in resource-limited environments.

==> sections/1_introduction_old.tex <==
\section{Introduction}

        \sachit{should we re-order para 1, 2 and 3 to highlight repetition-sparsity trade-off?}Despite significant strides in accuracy, the burgeoning complexity and resource demands of deep learning models pose challenges for their widespread adoption across a wide range of domains~\citep{Resnet, gpt3, 2015SpeechDNN, jain2022collossl, mandlekar2021matters}. 
        This requires the development of innovative techniques to enhance DNN efficiency during inference on edge devices.
        Two such techniques have been studied extensively: binarization and sparsity. Binarization, a form of quantization, results in weight repetition as only two values appear repeatedly in the weight tensor~\citep{courbariaux2015binaryconnect}. 
        This approach significantly trims the memory footprint of the weight tensor, thereby decreasing memory I/O during inference~\citep{ucnn}. In contrast, sparsity leads to zero weight values. Since anything multiplied by zero is zero, weight sparsity leads to \emph{ineffectual} multiplications~\citep{wu2021sparseloop}. This approach reduces memory I/O during inference by not reading activations that would be multiplied by zero weights~\citep{gong2020save}. Thus, both these techniques are geared towards reducing memory I/O during inference.
        
        DNN inference efficiency is usually achieved by leveraging either binarization or sparsity. Ternary introduces sparsity to binary by introducing an additional zero weight in conjunction to binary weights. Ternary was conceived with the reasonable assumption that transitioning from binary to ternary models would only minimally impact inference latency due to the effect of zero weights~\citep{li2016ternary}. However, advances in the contemporary hardware-software systems have revealed a substantial increase in latency during such transitions~\citep{prabhakar2021summerge, fu2022q}.\sachit{This work aims to perform faster inference on contemporary hardware-software systems while retaining model accuracy.}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/Screen Shot 2024-04-21 at 9.20.45 PM.png} % Adjust width as necessary
    \caption{\textbf{On the left:} The conventional, isolated approach where hardware-software systems and quantization methods are designed separately, resulting in being ignorant of repetition-sparsity trade-off, leading to inefficient inference. \textbf{On the right:} {The PLUM Framework}, a unified design framework, performs quantization-system co-design to exploit the repetition-sparsity trade-off, thereby enhancing computational efficiency.
    }
    \label{fig:fig1}
    % \vspace{-10pt}
\end{figure}

\sachit{We achieve efficient inference by leveraging the concept of \textit{repetition-sparsity trade-off}.}
\sout{The key insight of this work is the concept of the \textit{repetition-sparsity trade-off}.} This trade-off explains the inference inefficiency of binary and ternary weight quantization. A traditional binary network chooses maximization of weight repetition while being ignorant of weight sparsity, whereas a ternary network introduces weight sparsity at the expense of weight repetition. For instance, transitioning from binary to ternary networks increases the number of possible unique 3x3 2D filters from 512 ($2^9$) to 19683 ($3^9$). This makes it exponentially harder to extract efficiency using filter repetition.

\begin{wrapfigure}[30]{r}{0.5\textwidth}
% \vspace{-5pt}    
    \centering
    \includegraphics[width=0.9\linewidth]{figures/Screen Shot 2024-04-14 at 2.06.34 PM.png}
\caption{\textbf{PLUM vs. Prior-Art method for ResNet on ImageNet}: The pronounced spread indicates that {PLUM} holistically outperforms {prior-art method of partitioned design using binary quantization}. It retaines competitive accuracy and pushes the Pareto front, exhibiting a +3.5\% improvement when both methods employ a comparable number of effectual parameters. Moreover, our method enhances inference efficiency, achieving a 26\% speedup, doubling energy efficiency, and reducing density by 2.8x for the same backbone.\looseness=-1}
 \label{fig:wrap-plot}
\end{wrapfigure}

        
 The conventional approach to deploying efficient DNNs has largely been a two-stage process: training the DNN with binarization or ternarization~\citep{bai2018proxquant}, followed by formulating a system design that reduces memory I/O by leveraging both weight repetition and/or sparsity~\citep{ucnn}. This partitioned design approach has revealed a pitfall: increased memory I/O during inference due to the repetition-sparsity trade-off. However, recent advancements in DNN inference systems can now exploit repetition and sparsity to improve efficiency as shown in~\citep{prabhakar2021summerge, fu2022q}. To this end, this paper proposes
 {a quantization-system co-design framework} called {\textbf{PLUM} (\textbf{PLU}s-\textbf{M}inus) \textbf{Framework}} \sachit{as seen in Figure~\ref{fig:fig1}}. 
 {The objective of this framework is to demonstrate and leverage the existence of repetition-sparsity trade-off.}
{PLUM} re-imagines different levels of stack working together in synergy to enhance computational efficiency during inference while retaining the model's accuracy: 
 a) co-design with SOTA systems, 
{called \textit{{PLUM} kernels}}, 
 that exploit both repetition and sparsity during DNN inference; 
 b) it introduces \textit{{PLUM quantization called signed binarization,}} that cause sparsity without decreasing repetition;
 c) it offers insights \sout{for representation learning by introducing \textit{\sachit{PLUM} EDE} that influences}\sachit{on updating} latent full-precision weights during training to improve accuracy \sachit{along with distribution of quantized and latent full-precision after training}.
 This {co-design allows signed binary} to reap significant benefits of exploiting sparsity during DNN inference, as shown in ~\citep{wang2020sparsert, chen2019eyeriss}, while retaining benefits caused by repetition.\sachit{We demonstrate gains in efficiency with respect to latency on Intel CPUs.}\sachit{Write contributions on efficiency?}
        
\textcolor{black}{In this paper, we present the concept of repetition-sparsity trade-off along with the {PLUM} framework. While the former explains the inference inefficiency of binary and ternary weight quantization, the latter leverages (and thus proves) this insight to improve the efficiency of DNN inference. This results in collaborative co-design between different layers of the computational stack to enhance efficiency.} {{\sachit{As seen in Figure~\ref{fig:wrap-plot},} compared to classic partitioned design for binary, PLUM framework} improves inference efficiency (with respect to energy, latency, and throughput) and reduces model density to allow the use of bigger models, resulting in more accuracy.} Based on our analysis and empirical evidence, we envision that the {PLUM} framework has the potential to positively shape the evolution of more efficient and high-performing deep learning models.
